Dynamic Byzantine Reliable Broadcast [Technical Report]

Reliable broadcast is a communication primitive guaranteeing, intuitively, that all processes in a distributed system deliver the same set of messages. The reason why this primitive is appealing is twofold: (i) we can implement it deterministically in a completely asynchronous environment, unlike stronger primitives like consensus and total-order broadcast, and yet (ii) reliable broadcast is powerful enough to implement important applications like payment systems. The problem we tackle in this paper is that of dynamic reliable broadcast, i.e., enabling processes to join or leave the system. This property is desirable for long-lived applications (aiming to be highly available), yet has been precluded in previous asynchronous reliable broadcast protocols. We study this property in a general adversarial (i.e., Byzantine) environment. We introduce the first specification of a dynamic Byzantine reliable broadcast (DBRB) primitive that is amenable to an asynchronous implementation. We then present an algorithm implementing this specification in an asynchronous network. Our DBRB algorithm ensures that if any correct process in the system broadcasts a message, then every correct process delivers that message unless it leaves the system. Moreover, if a correct process delivers a message, then every correct process that has not expressed its will to leave the system delivers that message. We assume that more than $2/3$ of processes in the system are correct at all times, which is tight in our context. We also show that if only one process in the system can fail---and it can fail only by crashing---then it is impossible to implement a stronger primitive, ensuring that if any correct process in the system broadcasts or delivers a message, then every correct process in the system delivers that message---including those that leave.

==> sections/motivation.tex <==
\section{Motivation}
\label{sec:motivation}

Prior attempts at sharding cryptocurrency systems proved unsatisfying.
This is mostly due to the underlying coordination protocol which these systems employ---consensus.
In these systems, sharding allows to exploit the commutativity of unrelated operations.
For instance, a transfer from Alice to Bob is commutative with another transfer from Carol to Drake and can execute in parallel.
Nevertheless, if the parties involved in the first transfer (Alice and Bob) belong to separate shards, then a cross-shard coordination protocol is necessary to atomically commit this transfer across the two shards.
Unfortunately, the great majority of transfers in cryptocurrency systems are across (not within) shards.
For this reason, the cross-shard protocol poses problems.

In our consensusless approach, we avoid the need for cross-shard commitment.
Intuitively, commitment of a transfer across shards involves two separate steps.
These steps are asynchronous, hence avoiding the commit protocol.
The first step is sending the money: this happens when the broadcast protocol with the transfer details (which the sender initiates) terminates successfully.
The second step is receiving the money: this happens when the transfer recipient receives sufficient proofs (from witnesses of the sender) that the transfer succeeded.
The recipient obtains this information non-interactively.

The cross-shard commit protocol is not only a performance issue, but also a potential avenue for attack, e.g., in OmniLedger where Byzantine users can exploit this protocol to freeze transactions [RapidChain].

% as opposed to full replication, a sharded design allows the capacity (throughput) of a replicated system to scale with the number nodes.

% blockchain based apps need, by design, to involve the whole set of parties. subsets (e. g. quorums) are not really an option.
% systems like pbft and descendants match this requirement

% overwhelming number of transactions cross the boundaries of shards in a sharded design [RapidChain S.5]
% a notable challenge in sharded designs for asset transfer is the requirement of an atomic cross-shard coordination protocol [omniledger, rapidchain, all other... see S.2.2 in RapidChain]


==> sty/packages.tex <==
\usepackage{libertine}

\usepackage{amsmath,amsfonts,amssymb,amsthm}
\usepackage{chngcntr}

\usepackage{datetime}
\usepackage{url}

% \usepackage{authblk}

\usepackage{lastpage}

\usepackage{natbib}
\setlength{\bibsep}{0.0pt}

%%% page setup

\usepackage[noheadfoot,left=.75in,right=.75in,top=1in,bottom=1in,
            columnsep=0.33in
            ]{geometry}
\setlength{\textheight}{9.0in}
\setlength{\columnsep}{0.33in}
\setlength{\textwidth}{7in}

\setlength{\topmargin}{0.0in}
\setlength{\headheight}{0.0in}
\setlength{\headsep}{0.0in}

%%% page setup

\usepackage[font=small,labelfont=bf,justification=centering]{caption}


% \usepackage[activate={true,nocompatibility},final,tracking=true,kerning=true,spacing=true,factor=1100,stretch=10,shrink=10]{microtype}
% \microtypecontext{spacing=nonfrench}

\usepackage{amssymb,amsmath,amsthm}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{definition}{Definition}
\newtheorem{notation}{Notation}
\newtheorem{property}{Property}

\usepackage[colorlinks=true,
            citecolor=blue,
            linkcolor=magenta]{hyperref}

% Cross-references using section sign (§)
\usepackage{cleveref}
\crefname{section}{\S}{\S\S}
\Crefname{section}{\S}{\S\S}
\crefformat{section}{\S#2#1#3}

\Crefname{assumption}{Assumption}{Assumptions}
\Crefname{property}{Property}{Properties}


%% For including pdf graphs
\usepackage{graphicx}

%% For dashed lines in tables
\usepackage{arydshln}

%% For merged rows in tables
\usepackage{multirow}

\usepackage{threeparttable}

\usepackage{paralist}

\usepackage[subtle]{savetrees}



